NetBooster: Empowering Tiny Deep Learning By Standing on the Shoulders of Deep Giants

Tiny deep learning has attracted increasing attention driven by the substantial demand for deploying deep learning on numerous intelligent Internet-of-Things devices. However, it is still challenging to unleash tiny deep learning's full potential on both large-scale datasets and downstream tasks due to the under-fitting issues caused by the limited model capacity of tiny neural networks (TNNs). To this end, we propose a framework called NetBooster to empower tiny deep learning by augmenting the architectures of TNNs via an expansion-then-contraction strategy. Extensive experiments show that NetBooster consistently outperforms state-of-the-art tiny deep learning solutions.

==> Sections/4-Experiments_bak.tex <==
\section{Experiments}
% In this section, we first introduce our experiment setup (Sec.~\ref{sec:exp-setup}), benchmark experiment results on representative datasets (Sec.~\ref{sec:exp-cifar} and Sec~\ref{sec:exp-image}). Then we perform detailed ablation studies of the proposed NetBooster framework to better understand the expansion and contraction step (Sec.~\ref{sec:exp-loc}, Sec.~\ref{sec:exp-ratio}, Sec.~\ref{sec:exp-decay}). 



\subsection{Experiment Setup}
\label{sec:exp-setup}
\textbf{Networks, datasets, and baselines. } We consider \uline{seven networks}, including three manually designed efficient networks (MobileNet-V2~\cite{sandler2018mobilenetv2} at different scales), one NAS-based efficient network (MCUNet~\cite{lin2020mcunet}), and three widely used ResNet-based networks~\cite{he2016deep}, on \uline{two representative image classification datasets} (i.e., ImageNet and CIFAR-100) to provide a thorough evaluation of the proposed NetBooster. 
\uline{Baselines:} We benchmark the proposed NetBooster over vanilla networks under standard training, a series of SOTA KD algorithms (i.e., KD~\cite{hinton2015distilling}, CC~\cite{peng2019correlation}, RKD~\cite{park2019relational}, AB~\cite{heo2019knowledge}, tf-KD~\cite{yuan2020revisiting}, RCO-KD~\cite{jin2019knowledge}, RocketLaunch~\cite{zhou2018rocket}, and CRD~\cite{tian2019contrastive}), and NetAug~\cite{cai2021network}, which is the pioneering work aiming at  boosting TNN training performance. 


\noindent \textbf{Training settings.} We develop our training settings based on the commonly adopted  settings for CIFAR-100~\cite{tian2019contrastive} and ImageNet~\cite{cai2021network}. Specifically, on \uline{CIFAR-100}, we train the expanded network for 240 epochs using an SGD optimizer with a batch size of 64, an initial learning rate of 0.1 decayed by 0.1 at the 150-th, 180-th, and 210-th epochs. In PLT, we decay the non-linear activation function in expanded blocks for 50 epochs and further finetune for 190 epochs. On \uline{ImageNet}, we train the expanded network for 160 epochs using an SGD optimizer with a batch size of 1024 and an initial learning rate of 0.2 with the cosine anneal learning rate decay. In PLT, we decay the non-linear activation function in expanded blocks for 40 epochs and further finetune for 110 epochs. 

\begin{table}{r}{0.6\textwidth}
    \centering
    \vspace{-3em}
    \caption{Benchmarking on CIFAR-100.}
    \vspace{1em}
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c|cc|cc|c}
    \toprule[2pt]
        Network & FLOPs & Params & Teacher & Training Method & Accuracy \\
        \midrule
        % \multirow{7}{*}{MobileNetV2} & \multirow{7}{*}{7.58M} & \multirow{7}{*}{0.81M} & - & Vanilla & 64.6 \\
        % &  &  & ResNet-50 & KD~\cite{hinton2015distilling} & 67.3 \\
        % &  &  & ResNet-50 & CRD~\cite{tian2019contrastive} & 69.1 \\
        % &  &  & VGG13 & KD~\cite{hinton2015distilling} & 67.3 \\
        % &  &  & VGG13 & CRD~\cite{tian2019contrastive} & 69.7 \\ 
        % &  &  & - & NetBooster & \\
        % &  &  & ResNet-50 & NetBooster+KD & \\
        % \midrule
        \multirow{8}{*}{ResNet-20} & \multirow{8}{*}{41.6M} & \multirow{8}{*}{0.28M} & - & Vanilla & 69.0 \\
        % &  &  & ResNet-56 & KD~\cite{hinton2015distilling} & 70.6 \\
        &  &  & ResNet-110 & KD~\cite{hinton2015distilling} & 70.6 \\
        % &  &  & ResNet-56 & CC~\cite{peng2019correlation} & 69.6\\
        &  &  & ResNet-110 & CC~\cite{peng2019correlation} & 69.4\\
        % &  &  & ResNet-56 & RKD~\cite{park2019relational} & 69.6 \\ 
        &  &  & ResNet-110 & RKD~\cite{park2019relational} & 69.2 \\ 
        % &  &  & ResNet-56 & AB~\cite{heo2019knowledge} & 69.4 \\ 
        &  &  & ResNet-110 & AB~\cite{heo2019knowledge} & 69.5 \\ 
        % &  &  & ResNet-56 & CRD~\cite{tian2019contrastive} & 71.1 \\ 
        &  &  & ResNet-110 & CRD~\cite{tian2019contrastive} & 71.4 \\ 
        &  &  & - & NetBooster & \textbf{69.4}\\ 
        % &  &  & ResNet-56 & NetBooster+KD & \textbf{} \\ 
        &  &  & ResNet-110 & NetBooster+KD & \textbf{71.6} \\ 
        \midrule
        \multirow{6}{*}{ResNet32} & \multirow{6}{*}{70.7M} & \multirow{6}{*}{0.47M} & - & Vanilla & 72.2 \\
        &  &  & ResNet110 & KD~\cite{hinton2015distilling} &  73.0 \\
        &  &  & ResNet110 & CC~\cite{peng2019correlation} & 71.4\\
        &  &  & ResNet110 & RKD~\cite{park2019relational} & 71.8 \\ 
        &  &  & ResNet110 & AB~\cite{heo2019knowledge} & 70.9 \\ 
        % &  &  & ResNet110 & CRD~\cite{tian2019contrastive} & 73.4 \\ 
        &  &  & - & NetBooster & \textbf{72.7}\\ 
        &  &  & ResNet110 & NetBooster+KD & \textbf{73.4} \\ 
        \bottomrule[2pt]
    \end{tabular}
    }
    \vspace{-2em}
    \label{tab:cifar}
\end{table}
\subsection{Benchmarking on CIFAR-100}
\label{sec:exp-cifar}
We first apply NetBooster to train ResNet-based networks on CIFAR-100 and benchmark with SOTA knowledge distillation based methods on ResNet-20 and ResNet-32. 
In particular, we validate the performance of NetBooster, as well as the effectiveness of combining the NetBooster with KD~\cite{hinton2015distilling} algorithms to marry the merits of both.
As shown in Table~\ref{tab:cifar}, \uline{(1)} directly applying NetBooster can lead to 0.4\% $\sim$ 0.5\% accuracy improvements over the vanilla ResNet-20 and ResNet-32 and even surpass some of the KD algorithms without the need to introduce additional guidance from larger networks (e.g.,  RKD~\cite{park2019relational} on ResNet-20 with ResNet-110 as the teacher network), indicating NetBooster can boost the learning ability of TNNs by augmenting TNNs to learn more complex features; and \uline{(2)} NetBooster can be combined with KD algorithms to achieve SOTA accuracy under the guidance from larger teacher networks. In particular, NetBooster with KD~\cite{hinton2015distilling} achieves up to a 2.6\% higher accuracy than the vanilla networks and surpass various KD algorithms by 0.2\% $\sim$ 2.5\%. The above observations validate that (1) NetBooster can be applied to augment TNNs as a plug-and-play module to boost the TNN's performance, and (2) it can be easily integrated with existing KD algorithms to further boost the performance. 



\begin{table}{R}{0.6\textwidth}
    \centering
    \vspace{-3.5em}
    \caption{Benchmarking on ImageNet. 'r' is the input resolution.}
    \vspace{1em}
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c|cc|cc}
    \toprule[2pt]
        Network  & FLOPs & Params & Training Method & Accuracy \\
        \midrule
        \multirow{7}{*}{\makecell[c]{MobileNetV2-Tiny\\(r=144)}} & \multirow{7}{*}{23.5M} & \multirow{7}{*}{0.75M} & Vanilla & 51.2 \\
        &  &  & RocketLaunch~\cite{zhou2018rocket} & 51.8 \\
        &  &  & tf-KD~\cite{yuan2020revisiting} & 51.9 \\
        &  &  & RCO-KD~\cite{jin2019knowledge} & 52.6 \\
        &  &  & NetAug~\cite{cai2021network} & 53.0 \\
        % &  &  & NetAug + KD & 54.4 \\ 
        &  &  & NetBooster &\textbf{ 53.7}\\
        % &  &  & NetBooster + KD & \textcolor{red}{\textbf{54.2}} \\
        \midrule
        \multirow{3}{*}{\makecell[c]{MCUNet\\(r=176)}} & \multirow{3}{*}{81.8M} & \multirow{3}{*}{0.74M} & Vanilla & 61.4 \\
        &  &  & NetAug~\cite{cai2021network} & 62.5 \\
        &  &  & NetBooster &\textbf{ 62.8}\\
        \midrule
        \multirow{3}{*}{\makecell[c]{MobileNetV2-50\\(r=160)}} & \multirow{3}{*}{50.2M} & \multirow{3}{*}{1.95M} & Vanilla & 61.4\\
        &  &  & NetAug~\cite{cai2021network} & 62.5\\
        &  &  & NetBooster & \textbf{62.7}\\
        \midrule
        \multirow{3}{*}{\makecell[c]{MobileNetV2-100\\(r=160)}} & \multirow{3}{*}{154.1M} & \multirow{3}{*}{3.47M} & Vanilla & 69.6\\
        &  &  & NetAug~\cite{cai2021network} & 70.5 \\
        &  &  & NetBooster & \textbf{70.9} \\
        \bottomrule[2pt]
    \end{tabular}
    }
    \vspace{-2em}
    \label{tab:imagenet}
\end{table}
\subsection{Benchmark on ImageNet}
\label{sec:exp-image}
To further evaluate the effectiveness of NetBooster, we benchmark NetBooster on the more challenging ImageNet dataset with NetAug~\cite{cai2021network} and various of KD algorithms (i.e., RocketLaunch~\cite{zhou2018rocket}, tf-KD~\cite{yuan2020revisiting}, and RCO-KD~\cite{jin2019knowledge}) using multiple variants of MobileNetV2~\cite{sandler2018mobilenetv2} including MobileNetV2-Tiny~\cite{cai2018proxylessnas}, MobileNetV2-50/100~\cite{sandler2018mobilenetv2}, and MCUNet~\cite{lin2020mcunet}. 
As shown in Table~\ref{tab:imagenet}, NetBooster achieves 1.3\% $\sim$ 2.5\% accuracy improvements over the vanilla networks, showing the strong ability on boosting the TNN accuracy by standing on the shoulder of deep giants generated by NetBooster. 

Compared with the KD baselines, our proposed NetBooster achieves 0.9\% $\sim$ 1.1\% accuracy improvement without the guidance from the teacher network, suggesting that the network expansion in NetBooster can equip the expanded network with sufficient capacity to effectively learn the complex features at least comparable with the large-scale teacher DNN used in the KD baselines, and the learned features can be effectively inherited by the target network from the PLT step. 

\begin{table}{r}{0.4\textwidth}
    \centering
    \vspace{-3em}
    \caption{Evaluating NetBooster's performance on ResNet-50. }
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c}
    \toprule[2pt]
       Network & Training method & Accuracy\\
       \midrule
       \multirow{3}{*}{ResNet-50} & Vanilla & 77.6 \\
       & NetAug~\cite{cai2021network} & 76.5 \\
       & NetBooster & \textbf{78.0} \\
       \bottomrule[2pt]
    \end{tabular}
    }
    \label{tab:resnet50}
    \vspace{-2em}
\end{table}
Compared with NetAug~\cite{cai2021network}, which is a pioneering work focusing on the similar scenario as NetBooster, we also achieve consistently superior performance over their method, suggesting the multi-dimensional network expansion and the PTL for features inheritance are more effective than the network width expansion and directly drop augmented neuron after training proposed in NetAug. It is worth noticing that, even training NetAug with two times of training epochs, NetBooster still achieves 0.3\% higher accuracy than NetAug (53.7\% v.s. 53.4\%). 

To evaluate how our proposed NetBooster works with larger DNNs, we further evaluate our NetBooster with ResNet-50~\cite{he2016deep}. As shown in Table~\ref{tab:resnet50}, NetBooster can still achieve superior performance with 0.4\% accuracy higher than the vanilla network, proving the NetBooster, although designed for boosting TNNs, can be considered as a general technique to boost various networks' performance. It is worth noticing that the NetAug suffers from an accuracy drop when applied on relatively larger DNNs (i.e., ResNet-50). 


% \subsection{Benchmark with Existing Training Methods on CIFAR}

\subsection{Ablation Study on $\mathcal{Q}1$}
\begin{table}{r}{0.5\textwidth}
    \centering
    \vspace{-6em}
    \caption{Ablation study on \textbf{what kind of block} to insert.}
    % \vspace{-1em}
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{c|ccc}
    \toprule[2pt]
    Inserted Block Type & Expanded Acc. & Final Acc. \\
    \midrule 
    Vanilla & - & 51.20 \\ 
    \midrule
        Inverted Residual & 54.90 & 53.70\\ 
        Basic Block & 54.52 & 53.41 \\
        Bottleneck Block & 55.23 & 53.62 \\
        \bottomrule[2pt]
    \end{tabular}}
    \label{tab:block to insert}
    \vspace{-2.5em}
\end{table}
We first validate our argument on what block to insert in the TNN proposed in Sec.~\ref{sec:method-expansion}. We use MobileNetV2-Tiny and ImageNet to evaluate the difference when using different expansion blocks. As shown in Table~\ref{tab:block to insert}, (1) NetBooster consistently achieves 2.21\%$~sim$2.50\% higher performance than the vanilla network baseline with different kinds of blocks to insert, and (2) although the inverted residual block we used does not have the highest expanded accuracy, but it can best inherit the learned features and thus best benefit the TNN training. 

\subsection{Ablation Study on $\mathcal{Q}2$}
\label{sec:exp-loc}

\begin{table}{r}{0.5\textwidth}
    \centering
    \vspace{-3em}
    \caption{Ablation study on \textbf{which block} to expand. }
    % \vspace{1em}
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{c|cc|cc}
    \toprule[2pt]
        \multirow{2}{*}{Expansion} & \multicolumn{2}{c|}{Expanded} &\multirow{2}{*}{Expanded Acc.} & \multirow{2}{*}{Final Acc.}  \\
        & FLOPs & Params & & \\
        \midrule
        Vanilla & 29.4M & 0.75M & - & 51.20 \\
        \midrule
        % Random Expand &  &  &  & \\
        Expand First 8 & 65.0M & 0.83M & 51.46 & 51.50 \\
        Expand Middle 8 & 49.6M & 0.93M & 52.98 & 52.62 \\
        Expand Last 8 & 51.2M & 1.25M & 53.90 & 52.47 \\
        % Uniform Expand &  &  &  53.25 & 51.30 \\
        \midrule
        Uniform Expand 8 & 63.9M & 0.99M & 54.90 & 53.70 \\
        \bottomrule[2pt]
    \end{tabular}
    }
    \vspace{-2em}
    \label{tab:block to expand}
\end{table}

To evaluate our arguments on where to expand in the TNNs proposed in Sec.~\ref{sec:method-expansion}, we perform ablation studies on trying to expand the network from different positions. We conduct our experiment with MobileNetV2-Tiny and ImageNet dataset. 


First, we evaluate \uline{which block} should we expand in the TNN. We consider four different settings in expansion, all with the same total number of expanded blocks. Specifically, we consider expanding the first, middle and last eight blocks and uniformly expanding one block in every two block as we do in NetBooster. 
As shown in Table~\ref{tab:block to expand}, uniformly expand achieves significantly higher accuracy (1.08\% $\sim$ 2.20\%) than the other settings. We suspect such results are because after contraction, the complex features learned by expansion blocks may be too much for a single layer to inherit, layers before and after the expanded layer also need to adjust correspondingly to better preserve the expanded network's performance. Thus, excessively stacking layers to be expanded together may fail the original network in inheriting the complex features. 


\begin{table}{r}{0.5\textwidth}
    \centering
    \vspace{-3em}
    \caption{Ablation study on \textbf{which layer} to expand in each block.}
    % \vspace{1em}
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{c|cc|cc}
    \toprule[2pt]
        \multirow{2}{*}{Expansion} & \multicolumn{2}{c|}{Expanded} &\multirow{2}{*}{Expanded Acc.} & \multirow{2}{*}{Final Acc.}  \\
        & FLOPs & Params & & \\
        \midrule
        Vanilla & 29.4M & 0.75M & - & 51.20 \\
        \midrule
        First Pointwise Conv &  63.9M & 0.99M & 54.90 & 53.70 \\
        Last Pointwise Conv & 156.0M & 2.46M &  58.59 & 52.99 \\
        Depthwise Conv & 42.4M & 0.82M & 53.75 & 52.72 \\
        \bottomrule[2pt]
    \end{tabular}
    }
    \vspace{-2em}
    \label{tab:layer to expand}
\end{table}

We further study expand \uline{which layer} in the inverted residual block achieves the optimal performance. As shown in Table~\ref{tab:layer to expand}, we exhaustively expand each of the layers in the inverted residual block and show that as we suggested in Sec.~\ref{sec:method-expansion}, uniformly expand layers in the network achieves the optimal performance with 1.08\% higher accuracy than expand depthwise convolution and 1.23\% $\sim$ 2.20\% higher accuracy than expand pointwise convolution layers. 


% \begin{table}{r}{0.7\textwidth}
%     \centering
%     \vspace{-3em}
%     \caption{Ablation study on \textbf{number of expansion layers and expansion ratio} of the network.}
%     \vspace{1em}
%     \resizebox{0.7\textwidth}{!}{
%     \begin{tabular}{cc|cc|cc}
%     \toprule[2pt]
%         \multirow{2}{*}{\# Layer} & \multirow{2}{*}{Ratio} & \multicolumn{2}{c|}{Expanded} &\multirow{2}{*}{Expanded Acc.} & \multirow{2}{*}{Final Acc.}  \\
%         & & FLOPs & Params & & \\
%         \midrule
%         \multicolumn{2}{c|}{Vanilla} & 29.4M & 0.75M & - & 51.20 \\
%         \midrule
%         4 & 4 & 43.6M & 0.79M & 52.67 & 53.07\\
%         8 & 4 & 50.7M & 0.90M & 53.43 & 53.48 \\
%         12 & 4 & 57.9M & 0.99M & 51.95 & 50.73 \\
%         4 & 6 & 52.4M & 0.82M & 53.95 & 53.80 \\
%         8 & 6 & 63.9M & 0.99M & 54.90 & 53.70 \\
%         12 & 6 & 75.6M & 1.14M & 53.63 & 52.31 \\
%         4 & 8 & 61.1M & 0.85M & 53.66 & 53.60\\
%         8 & 8 & 77.1M & 1.09M & 53.91 & 52.43 \\
%         12 & 8 & 93.3M & 1.30M & 53.70 & 51.91 \\
%         \bottomrule[2pt]
%     \end{tabular}
%     }
%     \vspace{-3em}
%     \label{tab:expansion ratio}
% \end{table}



==> Sections/6-Supple.tex <==
% \section{Appendix}
% \section{Directly Apply NetBooster on Small-scale Dataset}
% % CIFAR exps 
% We first apply NetBooster to train ResNet-based networks on CIFAR-100 and benchmark with SOTA knowledge distillation based methods on ResNet-20 and ResNet-32. 
% In particular, we validate the performance of NetBooster, as well as the effectiveness of combining the NetBooster with KD~\cite{hinton2015distilling} algorithms to marry the merits of both.

% \begin{table}{r}{0.6\textwidth}
%     \centering
%     \vspace{-3em}
%     \caption{Benchmarking on CIFAR-100.}
%     \vspace{1em}
%     \resizebox{0.6\textwidth}{!}{
%     \begin{tabular}{c|cc|cc|c}
%     \toprule[2pt]
%         Network & FLOPs & Params & Teacher & Training Method & Accuracy \\
%         \midrule

%         \multirow{8}{*}{ResNet-20} & \multirow{8}{*}{41.6M} & \multirow{8}{*}{0.28M} & - & Vanilla & 69.0 \\
%         % &  &  & ResNet-56 & KD~\cite{hinton2015distilling} & 70.6 \\
%         &  &  & ResNet-110 & KD~\cite{hinton2015distilling} & 70.6 \\
%         % &  &  & ResNet-56 & CC~\cite{peng2019correlation} & 69.6\\
%         &  &  & ResNet-110 & CC~\cite{peng2019correlation} & 69.4\\
%         % &  &  & ResNet-56 & RKD~\cite{park2019relational} & 69.6 \\ 
%         &  &  & ResNet-110 & RKD~\cite{park2019relational} & 69.2 \\ 
%         % &  &  & ResNet-56 & AB~\cite{heo2019knowledge} & 69.4 \\ 
%         &  &  & ResNet-110 & AB~\cite{heo2019knowledge} & 69.5 \\ 
%         % &  &  & ResNet-56 & CRD~\cite{tian2019contrastive} & 71.1 \\ 
%         &  &  & ResNet-110 & CRD~\cite{tian2019contrastive} & 71.4 \\ 
%         &  &  & - & NetBooster & \textbf{69.4}\\ 
%         % &  &  & ResNet-56 & NetBooster+KD & \textbf{} \\ 
%         &  &  & ResNet-110 & NetBooster+KD & \textbf{71.6} \\ 
%         \midrule
%         \multirow{7}{*}{ResNet32} & \multirow{7}{*}{70.7M} & \multirow{7}{*}{0.47M} & - & Vanilla & 72.2 \\
%         &  &  & ResNet110 & KD~\cite{hinton2015distilling} &  73.0 \\
%         &  &  & ResNet110 & CC~\cite{peng2019correlation} & 71.4\\
%         &  &  & ResNet110 & RKD~\cite{park2019relational} & 71.8 \\ 
%         &  &  & ResNet110 & AB~\cite{heo2019knowledge} & 70.9 \\ 
%         &  &  & ResNet110 & CRD~\cite{tian2019contrastive} & 73.1 \\ 
%         &  &  & - & NetBooster & \textbf{72.7}\\ 
%         &  &  & ResNet110 & NetBooster+KD & \textbf{73.4} \\ 
%         \bottomrule[2pt]
%     \end{tabular}
%     }
%     \vspace{-1.5em}
%     \label{tab:cifar}
% \end{table}


% As shown in Table~\ref{tab:cifar}, \uline{(1)} directly applying NetBooster can lead to 0.4\% $\sim$ 0.5\% accuracy improvements over the vanilla ResNet-20 and ResNet-32 and even surpass some of the KD algorithms without the need to introduce additional guidance from larger networks (e.g.,  RKD~\cite{park2019relational} on ResNet-20 with ResNet-110 as the teacher network), indicating NetBooster can boost the learning ability of TNNs by augmenting TNNs to learn more complex features; and \uline{(2)} NetBooster can be combined with KD algorithms to achieve SOTA accuracy under the guidance from larger teacher networks. In particular, NetBooster with KD~\cite{hinton2015distilling} achieves up to a 2.6\% higher accuracy than the vanilla networks and surpass various KD algorithms by 0.2\% $\sim$ 2.5\%. The above observations validate that (1) NetBooster can be applied to augment TNNs as a plug-and-play module to boost the TNN's performance, and (2) it can be easily integrated with existing KD algorithms to further boost the performance. 


\section{NetBooster as a General Technique to Improve Network Performance}
\label{app:more model}
Existing works have shown that although larger networks normally suffer from over-fitting instead of under-fitting, increasing the network capacity can still lead to non-trivially performance improvement~\cite{liu2021swin,he2016deep,liu2021swin2}. To validate whether NetBooster has the potential as a general technique to boost neural networks' performance, we further validate the NetBooster on ResNet-50~\cite{he2016deep} and DeiT-Tiny~\cite{touvron2021training} on the ImageNet dataset with input resolution 224. 

\begin{table}[t]
    \centering
    % \vspace{-3em}
    \caption{Evaluating NetBooster's performance on ResNet-50 and DeiT-Tiny. }
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{c|c|c}
    \toprule
      Network & Training method & Accuracy\\
      \midrule
      \multirow{2}{*}{ResNet-50} & Vanilla & 77.6 \\
      & NetBooster & \textbf{78.0} \\
      \midrule
      \multirow{2}{*}{DeiT-Tiny} & Vanilla & 72.2 \\ 
      & NetBooster & \textbf{73.7} \\
      \bottomrule
    \end{tabular}
    }
    \label{tab:resnet50}
    % \vspace{-2em}
\end{table}

\textbf{Experiments setting}: We follow the training setting in~\cite{he2016deep} and~\cite{touvron2021training} to train ResNet-50 and DeiT-Tiny, respectively. We follow the proposed setting to expand 50\% of blocks in ResNet-50 and DeiT-Tiny uniformly. Specifically, for ResNet-50, we expand the first layer into the inverted residual block with a depthwise convolution kernel size of 3, expansion ratio 6 in the first layer in the selected blocks. For DeiT-Tiny, we expand the first fully connected layer in the feedforward network of the selected blocks into two fully connected layers with an expansion ratio of 6. We set $E_d$ to 20\% of the total training epochs. 

\begin{figure}[!t]
    % \vspace{-2em}
    \centering
    \includegraphics[width=0.5\linewidth]{Figures/expand_final_vis.pdf}
    % \vspace{-1em}
    \caption{Visualization of the expanded accuracy (i.e., the accuracy of the expanded network) and final accuracy when using different numbers of expand blocks with an expansion ratio 6. }
    \label{fig:expansion-vis}
    % \vspace{-4em}
\end{figure}

\textbf{Results}: As shown in Table~\ref{tab:resnet50}, NetBooster leads to 0.4\% higher accuracy over vanilla training on the large-scale DNN (i.e., ResNet-50) and 1.5\% higher accuracy over the attention-based vision transformer (i.e., DeiT-Tiny), showing its promising potential in boosting all DNNs' performance. 


\section{Number of Expansion Layers}
\label{app:number of layer}
The other factor that controls the deep giant's capacity is the number of expansion layers. We evaluate the relationship between the expansion ratio and the final performance on MobileNetV2-Tiny and the ImageNet dataset with an input resolution of 144. As shown in Fig.~\ref{fig:expansion-vis}, we observe that with various numbers of expansion layers, (1) networks boosted by the expansion-then-contraction strategy in NetBooster can constantly surpass the performance of vanilla networks, proving the NetBooster's effectiveness, (2) the expanded network performance (ExpandAcc.) increase first then decrease. We suspect the decrease in the expanded network accuracy is due to the overly deep network makes it challenging to train the network effectively, and (3) the boosted network performance (FinalAcc.) also has the increase-then-decrease pattern, validating our selected number of expansion layers. 





